Opportunistic Mutual Exclusion

Mutual exclusion is an important problem in the context of shared resource usage, where only one process can be using the shared resource at any given time. A mutual exclusion protocol that does not use information on the duration for which each process uses the resource can lead to sub-optimal utilization times. We consider a simple two-process mutual exclusion problem with a central server that provides access to the shared resource. We show that even in the absence of a clock, under certain conditions, the server can opportunistically grant early access to a client based on timing information. We call our new protocol opportunistic mutual exclusion. Our approach requires an extra request signal on each channel between client and server to convey extra information, and the server can grant early access based only on the order of events rather than through measuring time. We derive the handshaking specification and production rules for our protocol, and report on the energy and delay of the circuits in a 65nm process.

==> Midnight/dolines.tex <==
\ifx\DOLINES\relax\endinput\else\let\DOLINES=\relax\fi % \input only once
%
% dolines.tex: Meta-macros to separate arguments by newlines and by
%	       empty lines.
% version: 1.0  release: 15 April 1991
%
% copyright (c) 1991 Marcel R. van der Goot
%
% USAGE:
%   See the file dolines.doc
%   You need Midnight/loop.tex to use these macros.
%
% original: csvax.cs.caltech.edu [131.215.131.131] in pub/tex
%	    (use anonymous ftp). Also in various archives.
%
% Caltech, Pasadena  ---  Marcel van der Goot
%			  marcel@cs.caltech.edu
%			    Caltech 256--80
%			    Pasadena, CA 91125
%			    USA
%			    (818) 356--4603
%

% update history:
% version 1.0: This one.
%	release 15 April 1991: This one.
%	release 8 February 1991: Used \next instead of \do_next, which
%		occasionally conflicted with use of \next in other macros.

%%%%%% CODE: (you don't need to read this to use the macros)

\input Midnight/loop % CHANGE this filename to correspond to your installation

%%%%%%% Reading from a different file
% This is relatively simple, it can be done with a loop. The read function
% reads a single line (that is what \read does). A file that is being
% \read always ends with an empty line, therefore no test for eof(lines_in)
% is needed in the inner loop.
%
%	 while (!eof(lines_in))
%	   {
%	     read(lines_in, _ln);
%	     if (_ln != empty_ln)
%		{
%		  beforelines();
%		  do { everyline(_ln);
%		       read(lines_in, _ln);
%		  } while (_ln != empty_ln);
%		  afterlines();
%		}
%	   }
%

{\catcode`\^^M=12 \endlinechar=-1 % 12 = other
\catcode`\_=11 % 11 = letter (used to make macros private)

\newread\lines_in

\globaldefs=1

\def\empty_ln{\par}

\def\filedolines#1%
   {{\openin\lines_in=#1 %
     \ifeof\lines_in\message{File #1 not found.}\fi
     \Loop\ifeof\lines_in \Break1 \fi
          \read\lines_in to\_ln
          \ifx\_ln\empty_ln
          \else {\beforelines
	         \Loop\everyline{\_ln}%
		      \read\lines_in to\_ln
		      \ifx\_ln\empty_ln \Break1 \fi
	         \Pool
	         \afterlines
	        }%
          \fi
     \Pool
     \closein\lines_in
   }}

} % restore \catcode`\^^M, \catcode`\_, etc.


%%%%%%% Reading from the current file
% This is more complicated. The problem is that a line can only be
% read at the end of a macro, because otherwise a part of the macro
% itself will be read. Therefore, the above solution with \Loop cannot
% be used. Instead, this is implemented as a finite state machine. The
% FSM has two major states, outer_loop and inner_loop, corresponding to the
% program above. In these states, the value of _ln is used to determine
% what actions to take, and what the next state is. The next state
% is indicated by the control-sequence \do_next.
%    There are two minor states, get_out and get_in. In each of them
% the next line is read into _ln. After get_out, the next state is always
% outer_loop; after get_in it is always inner_loop.
%    Here is a ``picure.'' `(...)' is a state, `...?' denotes the value
% of _ln, and other texts are actions. ctrl-M stands for an empty line.
%
%				 /---<----\
%			    (get_out)	  |
%				 \      ctrl-M?
%   begindolines		  V      /
%     \->bgroup -> (get_out) -> (outer_loop) -> enddolines? -> egroup
%				 ^   |    ^		        \-> (finish)
%				/    |	   \
%		  afterlines --/   other?   \-- afterlines
%			^	     V		     ^
%			|	beforelines	     |
%	            ctrl-M? <--\     |      /--> enddolines?
%				\    V     /
%				(inner_loop)
%				  /     ^
%			     other?      \
%			      |        (get_in)
%			      V            |
%			      \-everyline->/
%


{\catcode`\^^M=12 \endlinechar=-1 % 12 = other
\catcode`\_=11 % 11 = letter (used to make macros private)
\globaldefs=1


\long\def\get_out#1^^M% here a line is read (as #1)
   {\gdef\_ln{#1}%
    \outer_loop
   }

\long\def\get_in#1^^M% here a line is read (as #1)
   {\gdef\_ln{#1}%
    \inner_loop
   }

\def\outer_loop
   {\ifx\_ln\enddolines \egroup\let\do_next=\finishdolines
    \else\ifx\_ln\empty \let\do_next=\get_out
    \else \beforelines\let\do_next=\inner_loop
    \fi  \fi
    \do_next
   }

\def\inner_loop
   {\ifx\_ln\enddolines \afterlines\let\do_next=\outer_loop
    \else\ifx\_ln\empty \afterlines\let\do_next=\outer_loop
    \else \everyline\_ln\let\do_next=\get_in
    \fi  \fi
    \do_next
   }

\def\begindolines
   {\bgroup
    \catcode`\^^M=12 %
    \get_out
   }

} % restore \catcode`\^^M, \catcode`\_, etc.

% We define \finishdolines and \enddolines, in case someone forgets:

\let\finishdolines=\relax
\def\enddolines{\enddolines}



==> Midnight/loop.tex <==
\ifx\LOOP\relax\endinput\else\let\LOOP=\relax\fi % \input only once
%
% loop.tex: A simple looping construct (meta-macros).
% version: 1.0  release: 26 June 1991
%
% copyright (c) 1991 Marcel R. van der Goot
%
% USAGE:
%   See the file loop.doc
%
% original: csvax.cs.caltech.edu [131.215.131.131] in pub/tex
%	    (use anonymous ftp). Also in various archives.
%
% Caltech, Pasadena  ---  Marcel van der Goot
%			  marcel@cs.caltech.edu
%			    Caltech 256--80
%			    Pasadena, CA 91125
%			    USA
%			    (818) 356--4603
%

% update history:
% version 1.0: This one.
%	release 26 April 1991: This one.
%	release 15 April 1991: Did not have \long in \Loop, \_break, and
%		\_continue.
%	release 8 Feb 1991: Used \next instead of \Lp_next.
%	

%%%%%% CODE: (you don't need to read this to use the macros)

{
\catcode`\_=11 % 11 = letter; to make macros private
\globaldefs=1

% Code to supply \fi's:

\def\do_fi{\fi\finish_ifs}

\def\finish_ifs
   {\ifnum\count255>0 %
	 \let\Lp_next=\do_fi
    \else\let\Lp_next=\relax
    \fi
    \advance\count255 by-1 %
    \Lp_next
   }

% The loop (tail-recursion does not clog memory):

\long\def\Loop#1\Pool%
   {\def\Pool{#1\Pool}%
    \Pool
   }

% \Break could have been defined as
%	\def\Break#1#2\Pool{{\count255=#1 \finish_ifs}}
% but this fails if you do
%	\ifnum\count0>5\Break
% without space after the 5: \Break wil be expanded to see if there
% are more digits (and expanding \Break means reading its 2nd argument).
% With the solution below, only \Break is expanded because it starts
% with \relax which is not a number. Using \afterassignment rather
% than passing the number as argument gives better error messages.

\def\Break
   {\relax\afterassignment\_break
    \bgroup\count255=
   }

\long\def\_break#1\Pool%
   {\finish_ifs
    \egroup
   }

\def\Continue
   {\relax\afterassignment\_continue
    \bgroup\count255=
   }

\long\def\_continue#1\Pool%
   {\finish_ifs
    \egroup
    \Pool
   }

} % restore \catcode`\_, \globaldefs



==> prs.tex <==
\ifx\PRS\UNDEFINED\let\PRS=\relax\else\endinput\fi % \input only once
%
% prs.tex: Macros for asynchronous vlsi.
% version: 2.0  release: 28 July 1995
%
% copyright (c) 1991, 1995 California Institute of Technology
% Author: Marcel R. van der Goot
%
% USAGE:
%   See the file prs.doc
%   You need Midnight/dolines.tex and Midnight/loop.tex to use these macros.
%
% Caltech, Pasadena  ---  Marcel van der Goot
%			  marcel@cs.caltech.edu
%			    Caltech 256--80
%			    Pasadena, CA 91125
%			    USA
%			    (818) 356-4603
%

% Update history:
%
% version 2.0: Some real improvements of the original.
%	release 28 July 1995: First version 2.0. Changes w.r.t. version 1.1
%		include: recognize [] in at-mode; slightly less space before
%		subscripts in @li@, @ro@; \noiosubscripts; @-@ as robust as
%		@+@; allow right-alignment of guards in prs; use LaTeX counter
%		for prs; \beginprs takes argument in TeX; page breaks possible
%		between groups in prs env; hse* and csp* envs; \defaboveprs;
%		better portability between macro packages (\prsstyle);
%		backquote for subscripts; roman numbers in at-mode; page
%		breaks in hse and csp envs; #; tabs invalid in hse;
%		internal name changes; some external name changes (he -> hse);
%		versions for NFSS1 and LaTeX2e. Also, doc was rewritten from
%		scratch.
% version 1.1: First distribution as part of CAST.
%	release 24 July 1995 - 26 Apr 1993: Individual changes no longer
%		recorded.
% version 1.0: The original.
%	release 26 Apr 1993 - 9 Dec 1991:  Individual changes no longer
%		recorded.
%       release 9 Dec 1991: The original
%

%%%%%% CODE: (you don't need to read this to use the macros)

\input Midnight/dolines % change this to the proper filename

\edef\PRS{\the\catcode`\_ }
\catcode`\_=11 % to make private macros

\newtoks\everyat % like \everymath

%%%%%%%%%% general %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\hexdigit#1% expands #1 (0<=#1<16) to single hex digit; can be used
   % when a number is needed, in particular for mathcodes.
   {\ifcase#1 0\or 1\or 2\or 3\or 4\or 5\or 6\or 7\or 8\or 9\or A\or B\or
              C\or D\or E\or F\fi
   }

% If for some reason \ttfam has changed (maybe in NFSS?), call \prsdeftt
% (If \tt does not select tt in mathmode for a package, then redefine
% \prsdeftt for that package --- see `macro packages' below.)
\def\prsdeftt
   {\setbox0=\hbox{$\tt\global\chardef\ttfam=\the\fam$}}


% \prs_it is supposed to switch to italic within math mode. Normally,
% \it works fine, but if it doesn't a macro package can redefine \prs_it.
% \prs_it is only used in math mode.

% \let\prs_it=\it % actual assignment is below under `defaults'

% The backquote is subscript character in at-mode, because underscores
% are letters in that mode. It is then easier if backquotes are also
% subscript characters in mathmode. They cannot be made subscript chars
% in general, because then you cannot print backquotes anymore; hence
% we use \everymath and \everydisplay.

\everymath=\expandafter{\the\everymath\catcode`\`=8 }
\everydisplay=\expandafter{\the\everydisplay\catcode`\`=8 }

\def\@{\char`\@}

%%%%%%%%%% at-mode %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% @ ... @ : Text between @ symbols is set as in math mode, but with the
%	changes described under \setup_at; also, text italic is used
%	rather than math italic.
% \useatmode : You may need to say this if the catcode of @ has been changed
%	(done by some macro packages, e.g., LaTeX).
% \setup_at : Define various characters and escape sequences with special
%	meaning in at-mode.
% \prsleftarrowfill, \prsrightarrowfill: for use in at-mode (unusual).

{% This is a bit tricky: in \setup_at we want to give definitions of the
 % form  \catcode`*=\active \def*{\prs_i}. However, to write `\def*', * must
 % be active when lexical scanning is done, i.e., when \setup_at is defined
 % rather than when it is expanded. So the \catcode`*=\active in the definition
 % is not sufficient: * must already be active when the definition is read.
 % Fine, we can do that: just make it active while the def is read. However,
 % instead of `*', we want to do this for `i', `o', etc.. But if we
 % make, e.g., `o' active while the definition is read, then the `o' in
 % `\catcode' is also active: that wouldn't work. The solution, a dirty trick,
 % is to define \uccode`*=`o, which says that an upper case `*' is an `o'.
 % Then we say \uppercase{\def*{\prs_o}}: This first tokenizes, which leads
 % to an active * being read. Then everything is converted to upper case, which
 % results in an active `o' instead. Then the active `o' is defined. This works
 % fine because within \uppercase{...} the only thing that can be converted
 % to upper case is the `*'.
 % Some symbols, like +, just correspond to some character. Others have
 % to check what comes next: - for ->, [ for [], i, and o. To do that, you
 % could make them active. However, instead of making them active, their
 % mathode is set to "8000. That is better, because it leaves i and o letters.
 % If, e.g., o is active, you cannot write \arrow; now you can.
 % Some macros which assume that - prints a dash may no longer work (\relbar
 % has been redefined so that \longrightarrow still works).

\catcode`\*=\active

\let\+=\relax % because \+ is an `outer' macro (stupid)

\gdef\setup_at
   {% math symbols that print in a special way (catcode 12 = other)
    \catcode`\+=12 \mathcode`\+="5222 % + = \uparrow, but class 5 (=closing)
    \catcode`\-=12 \mathcode`\-="8000 %
       \uccode`*=`- \uppercase{\let*=\prs_minus}% - = \prs_minus
    \catcode`\&=12 \mathcode`\&="225E % & = \wedge
    \catcode`\|=12 \mathcode`\|="225F % | = \vee
    \catcode`\~=12 \mathcode`\~="23A % ~ = \neg
    \catcode`\_=12 \mathcode`\_="8000 %
       \uccode`*=`_ \uppercase{\let*=\_}% _ = \_
    \catcode`\>=12 % -> = \prsarrow (or \hsearrow)
    \catcode`\*=12 \mathcode`\*="4\hexdigit\ttfam 2A % * = \tt *
    \catcode`\[=12 \mathcode`\[="8000 %
       \uccode`*=`[ \uppercase{\let*=\prs_loop }% [ = \prs_loop
    \catcode`\]=12 \mathcode`\]="5\hexdigit\ttfam 5D % ] = \tt ]
    \catcode`\#=12 \mathcode`\#="8000 %
       \uccode`*=`\# \uppercase{\let*=\prsprobe }% # = \prsprobe
    % special characters
    \catcode`\`=8 % ` = subscript character
    \prs_io_catcode % normally: \mathcode`i="8000 \mathcode`o="8000
       \uccode`*=`i \uppercase{\let*=\prs_i}% i = \prs_i
       \uccode`*=`o \uppercase{\let*=\prs_o}% o = \prs_o
    % escaped characters
    \mathchardef\+="202B % \+ = +
    \mathchardef\-="2200 % \- = -
    \mathchardef\*="220F % \* = \bullet
    \mathchardef\[="405B % \[ = \rm [
    \mathchardef\]="505D % \] = \rm ]
    \mathchardef\|="4\hexdigit\ttfam 7C % \| = \tt |
    % interaction with other things
    \let\relbar=\prs_relbar
    \everymath=\expandafter{\the\everymath\prs_it}%
    \at_numbers
    % user hook
    \the\everyat
   }

} % to delimit \catcode`\*=\active

% - = \prs_minus, which checks what comes next:
%    - = \downarrow (but class 5, i.e., closing)
%    -> = \prs_arrow

\def\prs_minus
   {\futurelet\next\prs_setminus}
\def\prs_setminus
   {\ifx>\next\let\next=\prs_arrow
    \else\let\next=\relax\mathchar"5223 % like \downarrow, but class 5
    \fi
    \next
   }
\def\prs_arrow>{\prsarrow} % user can redefine \prsarrow

% [ = \prs_loop, which checks what comes next:
%    [ = \tt [
%    [] = \prs_bar

\def\prs_loop
   {\futurelet\next\prs_setloop}
\def\prs_setloop
   {\ifx]\next\let\next=\prs_bar
    \else\let\next=\relax\mathchar"4\hexdigit\ttfam 5B % \tt [
    \fi
    \next
   }
\def\prs_bar]{\thick_bar}

\def\thick_bar
   {\hbox to\fontdimen2\textfont\ttfam{\hss\the\textfont\ttfam [$\!\!$]\hss}%
   }

% By default, \prsprobe takes an argument and draws a line over it. If
% you redefine it, it need not take an argument. Note: if you want it
% to be \#, say \mathchardef\prsprobe=`\# (\let\prsprobe=\# gets you in
% an infinite loop).

\let\prsprobe=\overline

% \pll is defined as a parallel bar symbol; normally, \| gives you this
% symbol, but at-mode redefines it. Also, we make it into a relation, to
% get better spacing.

\def\pll{\delimiter"326B30D }


% While in at-mode, the letters i and o behave as if they are active (i.e.,
% they have mathcode "8000): they are \prs_i and \prs_o, respectively.
% They check for the next character: if that is not a letter
% or number, a subscripted i or o is used; otherwise, a normal i or o is used.
% Note that in "ai_", the i will be subscripted; whether one wants that or
% not is open to discussion. This interpretation is chosen because the
% `bubble' program often turns an identifier "ai" into "ai_".

\def\prs_io_sub
   {\mathcode`i="8000 \mathcode`o="8000 }

% Some people want to switch the automatic subscripting off; personally,
% I think that looks horrible (you might as well set everything verbatim). - MR
\def\noiosubscripts
   {\let\prs_io_catcode=\relax}
\def\iosubscripts
   {\let\prs_io_catcode=\prs_io_sub}

\def\prs_i
   {\futurelet\next\prssub_i}
\def\prs_o
   {\futurelet\next\prssub_o}

\def\prssub_i{\prs_sub{\mathchar"7169 }} % real `i' (mathcode != "8000)
\def\prssub_o{\prs_sub{\mathchar"716F }} % real `o'

% After assigning \next to be equal to the next character, we need to
% know the charcode of that character. Unfortunately, it is not allowed
% to write \count255=`\next; in fact, the only way in which it seems
% possible to get the actual character corresponding to \next is by
% doing \meaning\next, a rather dirty trick. If you know that \next has
% catcode 12, then \meaning\next gives "the character 1" if \next is 1.

\def\prs_getcharcode#1 #2 #3\relax% to be used with \meaning
   {\count255=`#3\relax}

\def\prs_sub#1%
   {\ifcat a\next #1% followed by a letter
    \else\ifcat 1\next % followed by an `other' character
	 \expandafter\prs_getcharcode\meaning\next\relax
	 \ifnum\count255<`0 \sb{\mit{\mkern1mu#1}}% not a number
	 \else\ifnum\count255>`9 \sb{\mit{\mkern1mu#1}}% not a number
	 \else #1% followed by a number
	 \fi\fi
    \else\sb{\mit{\mkern1mu#1}}% followed by something else
    \fi\fi
   }

% \relbar is redefined to use \- instead of -, otherwise \longrightarrow
% starts with a down arrow. \rightarrowfill and \leftarrowfill have the
% same problem, but they are supposed to be used in text rather than
% math- or at-mode (they start with a $). Rather than redefining them
% every time when at-mode is entered, \prsrightarrowfill etc. are defined;
% it is unlikely that they are ever needed.

\def\prs_relbar{\mathrel{\smash\-}}

{\catcode`@=11 % letter
\gdef\prsrightarrowfill{$\m@th\mathord\-\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\mathord\-\mkern-2mu$}\hfill
  \mkern-7mu\mathord\rightarrow$}
\gdef\prsleftarrowfill{$\m@th\mathord\leftarrow\mkern-7mu%
  \cleaders\hbox{$\mkern-2mu\mathord\-\mkern-2mu$}\hfill
  \mkern-7mu\mathord\-$}
}

% \numbersrm makes digits of class 0 instead of 7, so that they are not
% affected by the current math font. \numbersvar undoes this.
% We use this because in at-mode \it is used, which we don't want
% to affect the digits. If you say (globally) \numbersrm, you'll have to
% say \numbersvar if you want to change the digit's font in mathmode
% (practically the only use for that is when you use oldstyle digits).
% If you say (globally) \numbersvar, you still get roman numbers in at-mode,
% because in that case at-mode does a local \numbersrm. This makes at-mode
% less efficient, but has the advantage of greater portability.

\def\num_specials
   {\do0\do1\do2\do3\do4\do5\do6\do7\do8\do9}

\def\numbersrm
   {\def\do##1{\mathcode`##1=`##1}%
    \let\at_numbers=\relax
    \num_specials
   }

\def\numbersvar
   {\def\do##1{\count255=28672
               \advance\count255 by`##1
               \mathcode`##1=\count255
              }%
    \let\at_numbers=\numbersrm
    \num_specials
   }

% In at-mode, @ changes to mathmode if necessary, and makes the above
% changes. The next @ terminates at-mode, and mathmode if necessary.

{% to delimit \catcode`@=\active
\catcode`@=\active

\gdef\useatmode{\catcode`@=\active \let@=\at_open}

\expandafter\gdef\expandafter\dospecials\expandafter{\dospecials\do \@}

\gdef\at_open
   {\begingroup
    \setup_at
    \ifmmode\let@=\at_close
    \else\let@=\at_mclose$%
    \fi
    \prs_it
   }
}% to delimit \catcode`@=\active

\let\at_close=\endgroup
\def\at_mclose{$\endgroup}



%%%%%%%%%% prs environment %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text in the prs environment is read line by line, one line
% for each production rule.
% The production rules are divided in groups separated by empty lines.
% The rules within a group are aligned on the arrows, which print as normal
% arrows. The rules are set in at-mode.
% There are several environments (see also below under `macro packages'):
%   prs : print one column
%   prs* : print one column, and number production rules
%   prs2 : print two columns; columns can only be split between groups
%   prs2* : print two columns, and number prod. rules
%

\newbox\prs_box % to collect all the groups
\newbox\leftprs_box % for two-column (prs2)
\newbox\rightprs_box % for two-column (prs2)
\newdimen\prsindent
\newdimen\prsmiddle

% Production rules are numbered with \prsnr. When the env is called,
% \prsnr is the number of the first pr minus 1. The counter is reset (to 0)
% with \resetprsnr at the end of the environment. (E.g., if you don't
% want to reset it, do \let\resetprsnr=\relax.) \theprs prints the number,
% \numberprs sets the number with extra space for the production rule.
% In LaTeX, the normal counter commands, as well as \label, can be used
% for the `prs' counter.

% Counter \prsnr is defined below, under `macro packages'.

\def\theprs{(\number\prsnr)} % print the number

\def\numberprs{\hbox to2em{\hss\smallrm\theprs\quad}} % as printed in prs env

\def\incrprsnr{\global\advance\prsnr by1 }
\def\resetprsnr{\global\prsnr=0 }

% Each group is made with \halign, to align at the arrow. The template
% used is \template_prs. The following templates are predefined.
% Note that you can bypass the template on a per-guard basis with \hfill.

\def\guardsleft{\let\template_prs=\templ_prs_left}
\def\guardsright{\let\template_prs=\templ_prs_right}
\def\guardscenter{\let\template_prs=\templ_prs_center}

\def\templ_prs_left
   {\strut$##$\hfil&${}\>\prsarrow\>##$\hfil}
\def\templ_prs_right
   {\strut\hfil$##$&${}\>\prsarrow\>##$\hfil}
\def\templ_prs_center
   {\strut\hfil$##$\hfil&${}\>\prsarrow\>##$\hfil}

% Each group is started by \before_prs and ended with \after_prs.
% \every_prs is applied to each line. The whole \halign is put in the
% body of macro \halign_prs. You cannot do the \halign directly (without
% first putting it in a macro), because \halign starts a new row of
% the table as soon as it encounters anything else than \omit, \noalign,
% or the closing brace, regardless of whether it is something that actually
% contributes horizontal material. Hence, when dolines is used to
% read the next line and compare it with \endprs (or so), \halign takes
% the read itself as the start of another row in the table. As a result,
% the alignment always ends with an extra row without production rules,
% but with a \strut. This whole problem is avoided by first defining
% \halign_prs.

% If there is no production rule (i.e., no arrow) no alignment is done
% and the text is set in an hbox. Hence, the text is set in the normal
% font and not in at-mode/math-mode. If you switch to mathmode, you'll
% get at-mode instead.

\def\set_noprs#1->%
   {\expandafter\def\expandafter\halign_prs\expandafter
	{\halign_prs\omit\strut\hbox{#1}\span\omit\hfil\cr}
   }

\def\number_prs
   {\incrprsnr
    \numberprs
   }

% set the part before the arrow.
\def\set_prs#1->#2\end_pr%
   {\def\tmp{#2}%
    \ifx\tmp\empty\set_noprs#1->% no arrow
    \else\expandafter\def\expandafter\halign_prs\expandafter
		{\halign_prs\nr_prs#1&}
	 \set_rightprs#2
    \fi
   }

% set the part after the arrow.
\def\set_rightprs#1->%
   {\expandafter\def\expandafter\halign_prs\expandafter{\halign_prs#1\cr}
   }

\def\every_prs#1%
   {\expandafter\set_prs#1->\end_pr}

% \before_prs_ inserts space between groups, but not before the first group.
\def\before_prs_{\def\before_prs_{\vskip\baselineskip}}

\def\before_prs
   {\before_prs_
    \def\halign_prs
       {\halign\bgroup\span\template_prs\cr}
   }

% With 1 column setting, \prsindent is inserted in front of each group.
% The groups are then set so that page breaks are possible between
% groups. With 2 columns, that cannot be done, because then you get the same
% separation between columns. There, the indent is inserted in front
% of the whole box. This way, everything is in a single box, and no
% page breaks are possible (that would be hard for two-column anyway).
% Also, see definition of \beforeprs below (and accompanying comment).

\def\after_prs
   {\expandafter\def\expandafter\halign_prs\expandafter
	{\halign_prs\egroup} % matches \halign\bgroup
    \hbox{\prs_one_indent\vbox{\halign_prs}}
    \penalty400
   }

\def\endprs_onecol
   {\egroup % \setbox\prs_box=\vbox\bgroup
    \unvbox\prs_box
    \prs_oldind
    \resetprsnr
    \afterprs
   }

\def\endprs_twocol
   {\egroup % \setbox\prs_box=\vbox\bgroup
    {\dimen0=\ht\prs_box
     \splittopskip=0pt \splitmaxdepth=30cm
     \vfuzz=30cm \vbadness=10000
     \Loop\setbox\rightprs_box=\copy\prs_box
	  \setbox\leftprs_box=\vsplit\rightprs_box to.5\dimen0
	  \setbox\leftprs_box=\vbox{\unvbox\leftprs_box}%
	  \ifdim\ht\leftprs_box<\ht\rightprs_box \else \Break1 \fi
	  \advance\dimen0 by2\baselineskip
     \Pool
     \dimen0=\ht\leftprs_box
     \setbox\rightprs_box=\vbox to\dimen0{\unvbox\rightprs_box \vfill}%
     \hbox{\kern\prsindent
	   \box\leftprs_box
	   \kern\prsmiddle
	   \box\rightprs_box
	  }%
    }%
    \prs_oldind
    \resetprsnr
    \afterprs
   }

\def\begin_prs#1#2% #1=1/2 for nr columns; #2=0/1 for numbering no/yes
   {\beforeprs
    \setbox\prs_box=\vbox\bgroup
	\setup_at
	\let\everyline=\every_prs
	\let\beforelines=\before_prs
	\let\afterlines=\after_prs
	\ifnum#1>1
	     \let\prs_one_indent=\relax
	     \let\end_prs=\endprs_twocol
	\else
	     \def\prs_one_indent{\kern\prsindent}
	     \let\end_prs=\endprs_onecol
	\fi
	\ifnum#2>0
	     \let\nr_prs=\number_prs
	\else
	     \let\nr_prs=\relax
	\fi
        \def_end_prs#1#2
        \begindolines
   }

% \beginprs calls \call_prs to check whether the next char is a `*', a `2', or
% something else. In case of a `2', the 2 is read and the next char is checked
% for a `*'. Note that we must do \setup_at first, so that catcode changes
% will work correctly. (In particular, `\beginprs ~a->b+' should work; but
% \setup_at usually changes the catcode of ~ from 13 to 12.)

%%%%%%%%%% hse and csp environments %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text in the hse and csp environments is set with the original line breaks
% and spacing (i.e., spaces are not ignored). Don't use tabs.
% The text is set in at-mode; -> prints \hsearrow instead of \prsarrow; spaces
% are as wide as in \tt. The csp environment is identical, except includes
% an implicit \noiosubscripts.
% There are several environments (see also below under `macro packages'):
%   hse : normal hse
%   hse* : number lines
%   csp : no automatic subscript i and o
%   csp* : number lines
%

{\catcode`\*=\active

\gdef\setup_hse
   {\catcode`\ =12 \mathcode`\ ="8000
	\uccode`*=`\ \uppercase{\def*{\kern\hse_space}} % ' ' = \kern\hse_space
    \set_hse_space
    \catcode9=15 % tab = invalid character
    \def\prs_arrow>{\hsearrow}
   }
} % to delimit \catcode`\*=\active

\newdimen\hse_space

% \set_hse_space sets \hse_space to the proper value. This is done every
% time you enter an hse or csp env, in case you have changed the size of
% the tt font.
\def\set_hse_space
   {\hse_space=\fontdimen2\textfont\ttfam
   }


% For numbering lines. Counter \hsenr is defined below, under
% `macro packages.'

\def\thehse{\number\hsenr} % print the number

\def\numberhse{\llap{\smallrm\thehse\quad}} % as printed in hse env

\def\incrhsenr{\global\advance\hsenr by1 }
\def\resethsenr{\global\hsenr=0 }

\def\number_hse
   {\incrhsenr
    \numberhse
   }

\def\every_hse#1%
   {\hbox \hselinewd{\hskip\prsindent\nr_hse\strut$\prs_it#1$\hfil}\penalty400}

% You can do:
%   \def\hselinewd{to\hsize}
% to make lines wider, thus enabling right alignment
% By default, lines are set at their natural width.
\def\hselinewd{}

\def\before_hse
   {\def\beforelines{\hbox{\strut}}%
   }
\let\after_hse=\relax

\def\end_hse
   {\egroup % \setbox\prs_box=\vtop\bgroup
    \unvbox\prs_box
    \prs_oldind
    \resethsenr
    \afterhse
   }   

\def\begin_hse#1#2% #1=0/1 for hse/csp; #2=0/1 for numbering no/yes.
   {\beforehse
    \setbox\prs_box=\vtop\bgroup
	\let\everyline=\every_hse
	\let\beforelines=\before_hse
	\let\afterlines=\after_hse
	\ifnum#1>0
	     \noiosubscripts
	\fi
	\ifnum#2>0
	     \let\nr_hse=\number_hse
	\else\let\nr_hse=\relax
	\fi
	\setup_at
	\setup_hse
	\def_end_hse#1#2
	\begindolines
   }


%%%%%%%%%% processes %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \defabove and \defleft can be used to put a process name at the beginning
% of the hse or csp environment.

\newbox\def_cspbox

% \defabove sort of works with hse*: no number is printed, but the number
% is incremented.
\def\defabove#1%
   {$\hfil\egroup\setbox\def_cspbox=\lastbox
    \hbox \hselinewd\bgroup\strut$\prs_it#1\equiv\prs_oldind
    \vrule depth1.5\dp\strutbox width0pt
   }

% \defaboveprs can be used with the prs env (but prs2 will look strange).
\def\defaboveprs#1%
   {\kern-\prsindent$\prs_it#1\equiv$\vrule depth1.5\dp\strutbox width0pt}

% We use \prs_oldind to restore the old value of \prsindent. If \prs_oldind
% is already defined (i.e., not \relax), we do not change it. This is
% all a bit cumbersome because \defleft is used inside a box, so assignments
% must be global.

% Use of \defleft is normally followed by a %, to wrap the line.

% \defleft omits the number, like \defabove.
\def\defleft#1%
   {$\hfil\egroup\setbox\def_cspbox=\lastbox
    \hbox \hselinewd\bgroup\strut$\prs_it
    \setbox\def_cspbox=\hbox{$#1\equiv\>$}%
    \ifx\prs_oldind\relax
	\xdef\prs_oldind
	   {\noexpand\global\noexpand\prsindent=\the\prsindent
	    \noexpand\global\noexpand\let\noexpand\prs_oldind=\noexpand\relax
	   }%
    \fi
    \global\prsindent=\wd\def_cspbox
    \copy\def_cspbox
   }

\let\prs_oldind=\relax


%%%%%%%%%% defaults %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% These could possibly be changed by a macro package; see \prsstyle below.

\everyat={}
\let\prsarrow=\rightarrow
\let\hsearrow=\longrightarrow

\prsindent=2\parindent
\prsmiddle=4em

\guardsleft

\iosubscripts

\numbersrm

\let\prs_it=\it

%%%%%%%%%% macro packages %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \prsstyle can be defined to include package specific definitions. If
% \prsstyle is not defined: if \documentstyle is defined, definitions
% for LaTeX are included, otherwise, definitions for plain TeX are included.
% (Note: when \prsstyle is expanded, \catcode`\_=11 (letter).)
% Of course, most definitions can also be changed after this file is
% included.

\ifx\prsstyle\UNDEFINED
     \ifx\documentstyle\UNDEFINED
          \def\prsstyle{\input prstex}
     \else\def\prsstyle{\input prslatex}
     \fi
\fi
\prsstyle

%%%%%%%%%% packages: environments

% If \prsstyle is defined, then it must define the following environments.
%
% prs:	Define prs, prs*, prs2, and prs2* environments, calling
%	\begin_prs with arguments 10, 11, 20, and 21, respectively.
%	You should also define a macro \def_end_prs#1#2, which, when called
%	with the same arguments, defines \enddolines and \finishdolines
%	appropriately. \finishdolines must call \end_prs. Also define
%	\beforeprs and \afterprs.
%
% hse:	Define hse and hse* environments, calling
%	\begin_hse with arguments 00 and 01 respectively.
%	You should also define a macro \def_end_hse#1#2, which, when called
%	with the same arguments, defines \enddolines and \finishdolines
%	appropriately. \finishdolines must call \end_hse. Also define
%	\beforehse and \afterhse.
%
% csp:  Define csp and csp* environments, calling
%	\begin_hse (!) with arguments 10 and 11 respectively. Otherwise,
%	the csp environment is identical to the hse environment, e.g.,
%	macro \def_end_hse is used to define \enddolines and \finishdolines.

%%%%%%%%%% packages: numbering

% For the prs* environment, the value of the counter is
% printed with \theprs, incremented with \incrprsnr, and reset with
% \resetprsnr. The counter itself is defined with \newcount\prsnr.
% You can change this in the file which is included. The \newcount
% is only done if the included file does not define \prsnr.
% Likewise for the hse* environment, except the names are
% \thehse, \incrhsenr, \resethsenr, and \hsenr. The csp* environment
% uses the same names as the hse* environment.
%

% Define \prsnr and \hsenr, if necessary.

\ifx\prsnr\UNDEFINED
     \newcount\prsnr
\fi

\ifx\hsenr\UNDEFINED
     \newcount\hsenr
\fi

%%%%%%%%%% packages: fonts

% \ttfam is used to refer to the math family containing font \tt, so that
% we can define mathchars refering to that font.
% You can set it with \prsstyle, but normally the following works just fine.

\ifx\ttfam\UNDEFINED
    \prsdeftt
\fi

% We use \smallrm to set the numbers for the prs* and hse* environments.
% If \smallrm is already defined, we don't do anything; else, if \small
% is defined, we'll use \small\rm instead; else, we check if the current
% font is cmr12 or cmr10 at11pt, in which case we use cmr10 at11pt or
% cmr10, respectively; else, we use cmr9.

% The extra \edefs are needed because \fontname produces characters with
% catcode 12, whereas \next of course is defined with real letters of
% catcode 11.
\def\chfnt#1\endcnfnt% use with \fontname as below
   {\def\tmp{#1}
    \edef\tmp{\meaning\tmp}
    \def\next{cmr10 at 11.0pt}\edef\next{\meaning\next}
    \ifx\tmp\next \font\smallrm=cmr10
    \else\def\next{cmr12}\edef\next{\meaning\next}
         \ifx\tmp\next \font\smallrm=cmr10 at11pt
         \else\font\smallrm=cmr9
	 \fi
    \fi
   }

\ifx\smallrm\UNDEFINED
     \ifx\small\UNDEFINED
	  \expandafter\chfnt\fontname\font\endcnfnt
     \else\def\smallrm{\small\rm}
     \fi
\fi


%%%%%%%%%% initialization %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% These should be at the end, after the package-dependent stuff.

\catcode`\_=\PRS

\resetprsnr
\resethsenr
\useatmode

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> prsl.tex <==
\ifx\PRS\relax\endinput\else\let\PRS=\relax\fi % \input only once
%
% prs.tex: Macros for asynchronous vlsi.
% version: 1.1  release: 2o July 1993
%
% copyright (c) 1991 California Institute of Technology
% author: Marcel R. van der Goot
%
% USAGE:
%   See the file prs.doc
%   You need Midnight/dolines.tex and Midnight/loop.tex to use these macros.
%
% Caltech, Pasadena  ---  Marcel van der Goot
%			  marcel@cs.caltech.edu
%			    Caltech 256--80
%			    Pasadena, CA 91125
%			    USA
%			    (818) 356--4603
%

% update history:
% version 1.1: First distribution as part of CAST.
%	release 20 Jul 1993: Added \helinewd so that by default lines in he
%		env have their natural width (see 15 Jul 1992).
%	release 26 Apr 1993: Changed use of \parindent to \prsindent, to
%		prevent problems with global changes in \defleft.
%		Also removed recognition of `#' as comment in prs environment.
% version 1.0: The original.
%	release 7 Oct 1992: Added \defabove and \defleft.
%	release 15 Jul 1992: Put line of he env in hbox to hsize, to allow
%		right alignment, if you really want that.
%	release 14 Jul 1992: Added \[ and \], and put \tt [ ] in at-mode.
%	release 13 Jul 1992: Changed init of \beforeprs etc. to give correct
%		vertical spacing in LaTeX.
%	release 10 Jul 1992: Defined \Bar to be able to use it outside he env.
%	release 7 Jul 1992: Added @ to \dospecials
%	release 14 Jan 1992: Added \prsarrow, \longprsarrow.
%	release 13 Jan 1992: Added use of \end_pr instead of `.'
%	release 12 Dec 1991: Changed he environment to produce a vtop, and
%		use \beforehe instead of \beforeprs
%	release 11 Dec 1991: Added \*, \+, and \-, and a csp environment.
%	release 10 Dec 1991: Added \it to \everymath in \setup_at (needed to
%		get \phantom right).
%       release 9 Dec 1991: The original
%

%%%%%% CODE: (you don't need to read this to use the macros)

\input Midnight/dolines % change this to the proper filename

\newtoks\everyat

\everyat=\expandafter{\number\catcode`\_} % to remember the catcode

\catcode`\_=11 % to make private macros


%%%%%%%%%% at-mode %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% @ ... @ : Text between @ symbols is set as in math mode, but with the
%	changes described under \setup_at; also, text italic is used
%	rather than math italic.
% \useatmode : You may need to say this if the catcode of @ has been changed
%	(done by some macro packages, e.g., LaTeX).
% \setup_at : Change &, |, ~, +, -, and -> to print the appropriate symbols;
%	change _ to print an underscore; define i and o to make subscripted
%	i and o at the end of identifiers.
% \prs_i, prs_o, \prssub_i, \prssub_o: make i and o subscripted (see below).
% 

{% This is a bit tricky: in \setup_at we want to give definitions of the
 % form  \catcode`*=\active \def*{\prs_i}. However, to write `\def*', * must
 % be active when lexical scanning is done, i.e., when \setup_at is defined
 % rather than when it is expanded. So the \catcode`*=\active in the definition
 % is not sufficient: * must already be active when the definition is read.
 % Fine, we can do that: just make it active while the def is read. However,
 % instead of `*', we want to do this for `i', `o', and `_'. But if we
 % make, e.g., `o' active while the definition is read, then the `o' in
 % `\catcode' is also active: that wouldn't work. The solution, a dirty trick,
 % is to define \uccode`*=`o, which says that an upper case `*' is an `o'.
 % Then we say \uppercase{\def*{\prs_o}}: This first tokenizes, which leads
 % to an active * being read. Then everything is converted to upper case, which
 % results in an active `o' instead. Then the active `o' is defined. This works
 % fine because within \uppercase{...} the only thing that can be converted
 % to upper case is the `*'.
 % In at-mode, i and o behave as if they are active, but they are not actually
 % made active: instead, their mathode is set to "8000. That is better,
 % because it leaves i and o letters. If, e.g., o is active, you cannot
 % write \arrow; now you can. However, - is made active, rather than to give
 % it mathcode "8000, because otherwise \longrightarrow doesn't work (rather
 % obscure, I admit).

\catcode`*=\active
\catcode`-=\active

\let\+=\relax % because \+ is an `outer' macro (stupid)

\gdef\setup_at
   {\catcode`\&=12 \mathcode`\&="225E % \wedge
    \catcode`\|=12 \mathcode`\|="225F % \vee
    \catcode`\~=12 \mathcode`\~="23A % \neg
    \catcode`\+=12 \mathcode`\+="5222 % like \uparrow, but class 5 (=closing)
    \catcode`\-=13 \let-=\at_minus
    \catcode`\[=12 \mathcode`\[="475B % \tt [
    \catcode`\]=12 \mathcode`\]="575D % \tt ]
    \mathcode`i="8000 \mathcode`o="8000 %
    \catcode`\_=13 %
    \mathchardef\*="220F % \bullet
    \mathchardef\+="202B \mathchardef\-="2200 % + and -
    \mathchardef\[="405B \mathchardef\]="505D % normal brackets.
    \uccode`*=`i \uppercase{\global\def*{\prs_i}}%
    \uccode`*=`o \uppercase{\global\def*{\prs_o}}%
    \uccode`*=`_ \uppercase{\global\let*=\_}%
    \everymath=\expandafter{\the\everymath\it}%
    \the\everyat
   }

} % to delimit \catcode`*=\active


\def\at_minus
   {\futurelet\next\at_setminus}
\def\at_setminus
   {\ifx>\next\let\next=\at_arrow
    \else\let\next=\relax\mathchar"5223 % like \downarrow
    \fi
    \next
   }
\def\at_arrow>{\prsarrow}


% While in at-mode, the letters i and o behave as if they are active (i.e.,
% they have mathcode "8000): they are \prs_i and \prs_o, respectively.
% They check for the next character: if that is not a letter
% or number, a subscripted i or o is used; otherwise, a normal i or o is used.
% Note that in "ai_", the i will be subscripted; whether one wants that or
% not is open to discussion. This interpretation is chosen because the
% `bubble' program often turns an identifier "ai" into "ai_".

\def\prs_i
   {\futurelet\next\prssub_i}
\def\prs_o
   {\futurelet\next\prssub_o}

\def\prssub_i{\prs_sub{\mathchar"7169 }} % real `i' (mathcode != "8000)
\def\prssub_o{\prs_sub{\mathchar"716F }} % real `o'

% After assigning \next to be equal to the next character, we need to
% know the charcode of that character. Unfortunately, it is not allowed
% to write \count0=`\next; in fact, the only way in which it seems
% possible to get the actual character corresponding to \next is by
% doing \meaning\next, a rather dirty trick. If you know that \next has
% catcode 12, then \meaning\next gives "the character 1" if \next is 1.
\def\at_getcharcode#1 #2 #3{`#3}% to be used with \meaning

\def\prs_sub#1%
   {\ifcat a\next #1% followed by a letter
    \else\ifcat 1\next % followed by an `other' character
	 {\count0=\expandafter\at_getcharcode\meaning\next\relax
	  \ifnum\count0<`0 {\mit\sb{#1}}% not a number
	  \else\ifnum\count0>`9 {\mit\sb{#1}}% not a number
	  \else #1% followed by a number
	  \fi\fi
	 }%
    \else{\mit\sb{#1}}% followed by something else
    \fi\fi
   }

% In at-mode, @ changes to mathmode if necessary, and makes the above
% changes. The next @ terminates at-mode, and mathmode if necessary.

{% to delimit \catcode`@=\active
\catcode`@=\active

\gdef\useatmode{\catcode`@=\active \let@=\at_open}

\expandafter\gdef\expandafter\dospecials\expandafter{\dospecials\do \@}

\gdef\at_open
   {\begingroup
    \setup_at
    \ifmmode\let@=\at_close
    \else\let@=\at_mclose$%
    \fi
    \it
   }
}% to delimit \catcode`@=\active

\let\at_close=\endgroup
\def\at_mclose{$\endgroup}



%%%%%%%%%% production rules %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text between \beginprs ... \endprs is read line by line, one line
% for each production rule.
% The production rules are divided in groups separated by empty lines.
% The rules within a group are aligned on the arrows, which print as normal
% arrows. The rules are set in at-mode.
%
% \beginprs ... : print one column
% \beginprs* ... : print one column, and number production rules
% \beginprs2 ... : print two columns; columns can only be split between groups
% \beginprs2* ... : print two columns, and number prod. rules
% In TeX, the termination is always by `\endprs'.
%

\newbox\leftprs_box
\newbox\rightprs_box
\newbox\prs_box
\newcount\prs_nr

\newdimen\prsindent

{\catcode`\-=\active

% If there is no production rule (i.e., no arrow), we do not want at-mode.
% We won't bother to reset everything, we'll just not start math-mode and
% we'll use the normal font. If you switch to mathmode, you'll get at-mode
% instead (except in \mit instead of \it).
\gdef\set_noprs#1#2->%
   {\setbox\leftprs_box=\vbox{\unvbox\leftprs_box
			      \hbox{#1#2\strut}
			     }
    \setbox\rightprs_box=\vbox{\unvbox\rightprs_box
			       \hbox{\strut}
			      }
   }

\gdef\set_prs#1->#2\end_pr%
   {\def\tmp{#2}%
    \ifx\tmp\empty\set_noprs#1->%
    \else\setbox\leftprs_box=\vbox{\unvbox\leftprs_box
			       \hbox{\strut$%
				     \ifnum\prs_nr>0 (\mit\number\prs_nr)\quad
					   \global\advance\prs_nr by1 %
				     \fi
				     \it#1$%
			      }}
	 \set_rightprs#2
    \fi
   }

\gdef\set_rightprs#1->%
   {\setbox\rightprs_box=\vbox{\unvbox\rightprs_box
			       \hbox{\strut$\it\quad\prsarrow\quad#1$}
			      }
   }

\gdef\every_prs#1%
   {\expandafter\set_prs#1->\end_pr}

} %\catcode`\-=\active

\let\before_prs_=\relax

\def\before_prs
   {{\setbox0=\box\leftprs_box \setbox0=\box\rightprs_box}
    \before_prs_
    \def\before_prs_{\vskip\baselineskip}
   }
	
\def\after_prs
   {\hbox{\box\leftprs_box \box\rightprs_box}\penalty-500}

\def\endprs_onecol
   {\egroup
    \hbox{\kern\prsindent\box\prs_box}
    \prs_oldind
    \afterprs
   }

\def\endprs_twocol
   {\egroup
    {\dimen0=\ht\prs_box
     \splittopskip=0pt \splitmaxdepth=30cm
     \vfuzz=30cm \vbadness=10000
     \Loop\setbox\rightprs_box=\copy\prs_box
	  \setbox\leftprs_box=\vsplit\rightprs_box to.5\dimen0
	  \setbox\leftprs_box=\vbox{\unvbox\leftprs_box}
	  \ifdim\ht\leftprs_box<\ht\rightprs_box \else \Break1 \fi
	  \advance\dimen0 by2\baselineskip
     \Pool
     \dimen0=\ht\leftprs_box
     \setbox\rightprs_box=\vbox to\dimen0{\unvbox\rightprs_box \vfill}
     \hbox{\kern\prsindent
	   \box\leftprs_box
	   \qquad\qquad
	   \box\rightprs_box
	  }
    }%
    \prs_oldind
    \afterprs
   }

\def\begin_prs#1#2*% 1/2 for nr columns, 0/1 for numbering
   {\beforeprs
    \setbox\prs_box=\vbox\bgroup
	\setup_at
	\catcode`\#=12
	\let\everyline=\every_prs
	\let\beforelines=\before_prs
	\let\afterlines=\after_prs
	\global\prs_nr=#2
	\ifnum#1>1
% IF TeX:
%	     \let\finishdolines=\endprs_twocol
% ELIF LaTeX:
	     \ifnum#2>0
		  \def\finishdolines{\end{prs2*}}
	     	  \def\enddolines{\end{prs2*}}
	     \else\def\finishdolines{\end{prs2}}
		  \def\enddolines{\end{prs2}}
	     \fi
% FI
	\else
% IF TeX:
%	     \let\finishdolines=\endprs_onecol
% ELIF LaTeX:
	     \ifnum#2>0
		  \def\finishdolines{\end{prs*}}
	     	  \def\enddolines{\end{prs*}}
	     \else\def\finishdolines{\end{prs}}
		  \def\enddolines{\end{prs}}
	     \fi
% FI
	\fi
% IF TeX:
%	\def\enddolines{\endprs}
% FI
        \begindolines
   }

% \beginprs calls \call_prs to check whether the next char is a `*', a `2', or
% something else. In case of a `2', the 2 is read and the next char is checked
% for a `*'.

% TeX, but no harm is done by defining it in LaTeX.

\def\beginprs{\futurelet\next\call_prs}

\def\call_prs
   {\ifx*\next\toks0={\begin_prs11}%
    \else\ifx2\next\toks0={\call_prstwo}%
    \else\toks0={\begin_prs10*}%
    \fi\fi
    \the\toks0 %
   }

\def\call_prstwo2{\futurelet\next\call_prstwob}
\def\call_prstwob
   {\ifx*\next\toks0={\begin_prs21}%
    \else\toks0={\begin_prs20*}%
    \fi
    \the\toks0 %
   }


%%%%%%%%%% handshaking expansions %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text between \beginhe ... \endhe is set in at-mode; * and [] are
% set in \tt; -> is longer than normal in at-mode; spaces are as wide as
% in \tt, and are not ignored.
%

{\catcode`\[=\active

\gdef\setup_he
   {\uccode`[=`\ \uppercase{\def[{\kern\he_space}}
    \catcode`\*=12 \catcode`\[=13 \catcode`\ =\active
    \mathcode`\*="472A % fam 7 = tt in plain TeX
    \let[=\he_do
    \def\at_arrow>{\longprsarrow}
    \mathchardef\|="477C
   }
}

\newdimen\he_space
\setbox0=\hbox{\tt *}
\he_space=\wd0

\def\he_do
   {\futurelet\next\he_dotest}

\def\he_dotest
   {\ifx]\next\let\next=\he_bar
    \else\let\next=\relax\mathchar"475B %
    \fi
    \next
   }

\def\he_bar]{\Bar}

\def\Bar
   {{\setbox0=\hbox{\tt *}%
     \hbox to\wd0{\hss\tt[$\!\!$]\hss}%
   }}

\def\every_he#1%
   {\hbox \helinewd{\hskip\prsindent\strut$\it#1$\hfil}}

\def\helinewd{}
% You can do:
%   \def\helinewd{to\hsize}
% to make lines wider, thus enabling right alignment

\def\before_he{\def\beforelines{\hbox{\strut}}}
\let\after_he=\relax

\def\end_he{\egroup\prs_oldind\afterhe}

\def\beginhe
   {\beforehe
    \vtop\bgroup
	\let\everyline=\every_he
	\let\beforelines=\before_he
	\let\afterlines=\after_he
% IF TeX:
%	\def\enddolines{\endhe}
%	\let\finishdolines=\end_he
% ELIF LaTeX:
	\def\enddolines{\end{he}}
	\def\finishdolines{\end{he}}
% FI
	\setup_at
	\setup_he
	\begindolines
   }

%%%%%%%%%% csp programs %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The csp environment is just like the he environment, except that the i and o
% do not print as subscripts.

\def\begincsp
   {\beforehe
    \vtop\bgroup
	\let\everyline=\every_he
	\let\beforelines=\before_he
	\let\afterlines=\after_he
% IF TeX:
%	\def\enddolines{\endcsp}
%	\let\finishdolines=\end_he
% ELIF LaTeX:
	\def\enddolines{\end{csp}}
	\def\finishdolines{\end{csp}}
% FI
	\setup_at
	\setup_he
	\mathcode`i="7169 \mathcode`o="716F
	\begindolines
   }


%%%%%%%%%% Processes %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\defabove#1%
   {\kern-\prsindent#1\equiv\prs_oldind
    \vrule depth5pt width0pt
   }

% We use \prs_oldind to restore the old value of \prsindent. If \prs_oldind
% is already defined (i.e., not \relax), we do not change it. This is
% all a bit cumbersome because \defleft is used inside a box, so assignments
% must be global.

\newbox\def_cspbox
\def\defleft#1%
   {\setbox\def_cspbox=\hbox{$#1\equiv\>$}%
    \kern-\prsindent
    \ifx\prs_oldind\relax
	\xdef\prs_oldind
	   {\noexpand\global\noexpand\prsindent=\the\prsindent
	    \noexpand\global\noexpand\let\noexpand\prs_oldind=\noexpand\relax
	   }%
    \fi
    \global\prsindent=\wd\def_cspbox
    \copy\def_cspbox
   }

\let\prs_oldind=\relax

%%%%%%%%%% LaTeX and initialization %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% IF LaTeX:
\newenvironment{he}{\beginhe}{\end_he}
\newenvironment{csp}{\begincsp}{\end_he}
\newenvironment{prs}{\begin_prs10*}{\endprs_onecol}
\newenvironment{prs*}{\begin_prs11*}{\endprs_onecol}
\newenvironment{prs2}{\begin_prs20*}{\endprs_twocol}
\newenvironment{prs2*}{\begin_prs21*}{\endprs_twocol}
\def\makeatother{\useatmode}
% FI

\catcode`\_=\the\everyat

% initialization:

\everyat={}
\let\prsarrow=\rightarrow
\let\longprsarrow=\longrightarrow

\prsindent=2\parindent


% IF TeX:
%\def\beforeprs{\endgraf\medskip}
%   % the endgraf isn't really needed
%\def\afterprs{\endgraf\medskip}
% ELIF LaTeX:
\def\beforeprs{\trivlist\item[]\leavevmode}
   % standard for LaTeX environments
\def\afterprs{\endtrivlist}
% FI
\let\beforehe=\beforeprs
\let\afterhe=\afterprs

\useatmode



==> prslatex.tex <==
% prstex.tex:
%	This file is loaded by prs.tex/prs.sty for use with
%	latex, latex2e, latex-nfss (=nfss1).
%	See prs.doc for documentation of the prs maros.
%
% copyright (c) 1995 California Institute of Technology
% Author: Marcel R. van der Goot

% Update history:
%
% version 2.0: For use with prs.tex version 2.0
%	release 26 July 1995: First version of this file (before, it was part
%		of prs.tex).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%% prs environment %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\let\tmp=\theprs
\newcounter{prs}
\def\incrprsnr{\refstepcounter{prs}}
\let\prsnr=\c@prs
\let\theprs=\tmp

{\catcode`\*=12 % because the * must be read in at-mode

\gdef\def_end_prs#1#2%
   {\ifnum#1>1
	 \ifnum#2>0
	      \def\enddolines{\end{prs2*}}
	 \else\def\enddolines{\end{prs2}}
	 \fi
    \else\ifnum#2>0
	      \def\enddolines{\end{prs*}}
	 \else\def\enddolines{\end{prs}}
	 \fi
    \fi
    \let\finishdolines=\enddolines
   }
}

\newenvironment{prs}{\begin_prs10}{\end_prs}
\newenvironment{prs*}{\begin_prs11}{\end_prs}
\newenvironment{prs2}{\begin_prs20}{\end_prs}
\newenvironment{prs2*}{\begin_prs21}{\end_prs}

% The spacing for environments in LaTeX is normally obtained with
% \trivlist\item[]\leavevmode. We need to pack the result in an extra vbox
% because in \endprs_onecol there's an \unvbox, which would cause a switch
% from horizontal to vertical mode, inserting a \par and extra space. You
% cannot omit the \leavevmode, because LaTeX will complain about a missing
% item. Note that the extra vbox prevents page breaks.

\def\beforeprs{\trivlist\item[]\leavevmode\vbox\bgroup}
\def\afterprs{\egroup\endtrivlist}

%%%%%%%%%% hse and csp environments %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\let\tmp=\thehse
\newcounter{hse}
\def\incrhsenr{\refstepcounter{hse}}
\let\hsenr=\c@hse
\let\thehse=\tmp

{\catcode`\*=12 % because the * must be read in at-mode

\gdef\def_end_hse#1#2%
   {\ifnum#1>0
	 \ifnum#2>0
	      \def\enddolines{\end{csp*}}
	 \else\def\enddolines{\end{csp}}
	 \fi
    \else\ifnum#2>0
	      \def\enddolines{\end{hse*}}
	 \else\def\enddolines{\end{hse}}
	      \he_compat % he environment, for compatibility.
	 \fi
    \fi
    \let\finishdolines=\enddolines
   }
}

\let\he_compat=\relax

\newenvironment{hse}{\begin_hse00}{\end_hse}
\newenvironment{hse*}{\begin_hse01}{\end_hse}

% for compatibility with the old version:
\newenvironment{he}{\typeout{WARNING: the he environment is now called hse}%
		    \def\he_compat{\def\enddolines{\end{he}}}%
		    \begin_hse00}%
		   {\end_hse}

\let\beforehse=\beforeprs
\let\afterhse=\afterprs

\newenvironment{csp}{\begin_hse10}{\end_hse}
\newenvironment{csp*}{\begin_hse11}{\end_hse}

%%%%%%%%%% other %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\makeatother{\useatmode}


% In LaTeX2e, \useatmode and \prsdeftt must be done after \begin{document}.
% Even if they have been done earlier, apparently \begin{document} resets
% them (in particular, the math families are only assigned when
% encountered). Luckily, LaTeX2e has a hook for this. We test for LaTeX2e
% by checking whether \documentclass is defined.

\ifx\documentclass\UNDEFINED
\else\message{[prs: latex2e]}
     \AtBeginDocument{\useatmode\prsdeftt}
\fi

% LaTeX2e uses release 2 of the NFSS. However, there are versions of LaTeX 2.09
% around which use release 1 of the NFSS. There, \tt doesn't change \fam,
% so we need to redefine \prsdeftt. We check for nfss1 by checking whether
% \new@internalmathalphabet is defined.

\ifx\new@internalmathalphabet\UNDEFINED
\else\message{[prs: latex-nfss1]}
     \ifx\ttfam\UNDEFINED
	  \new@mathgroup\ttfam
	  \new@internalmathalphabet\mathtt\ttfam{cmtt}{m}{n}
     \fi
     \ifx\itfam\UNDEFINED
	  \new@mathgroup\itfam
	  \new@internalmathalphabet\mathit\itfam{cmr}{m}{it}
     \fi
     {\setbox0=\hbox{$\mathit{x}$}}
     \def\prs_it{\fam=\itfam}
     \def\prsdeftt{\setbox0=\hbox{$\mathtt{x}$}}
     \prsdeftt
\fi

% LaTeX2e defines \oldstylenums{#1} for setting old style digits. We redefine
% it to include a \numbersvar. For other versions of LaTeX, we first
% define \oldstylenums. (Note: in nfss1, \mit takes an argument.)

\ifx\oldstylenums\UNDEFINED
	\def\oldstylenums#1{\ifmmode{\mit{#1}}\else$\mit{#1}$\fi}
\fi
\let\_oldstylenums=\oldstylenums
\def\oldstylenums#1{{\numbersvar\_oldstylenums{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> prstex.tex <==
% prstex.tex:
%	This file is loaded by prs.tex/prs.sty for use with
%	plain tex.
%	See prs.doc for documentation of the prs maros.
%
% copyright (c) 1995 California Institute of Technology
% Author: Marcel R. van der Goot

% Update history:
%
% version 2.0: For use with prs.tex version 2.0
%	release 26 July 1995: First version of this file (before, it was part
%		of prs.tex).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%% prs environment %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In TeX, use \beginprs{}, \beginprs{*}, \beginprs{2}, \beginprs{2*};
% always end with \endprs.

\def\beginprs#1%
   {\csname prs#1\endcsname
   }

\def\def_end_prs#1#2%
   {\def\enddolines{\endprs}
    \def\finishdolines{\end_prs}
   }

\def\prs{\begin_prs10}
\expandafter\def\csname prs*\endcsname{\begin_prs11}
\expandafter\def\csname prs2\endcsname{\begin_prs20}
\expandafter\def\csname prs2*\endcsname{\begin_prs21}

\def\beforeprs{\endgraf\medskip} % the endgraf isn't really needed
\def\afterprs{\endgraf\medskip\noindent}


%%%%%%%%%% hse and csp environments %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In TeX, use \beginhse{}, \beginhse{*}, \begincsp{}, \begincsp{*};
% end with \endhse for hse and hse*, with \endcsp for csp and csp*.

\def\beginhse#1%
   {\csname hse#1\endcsname
   }

\def\begincsp#1%
   {\csname csp#1\endcsname
   }

\def\def_end_hse#1#2%
   {\ifnum#1>0
	 \def\enddolines{\endcsp}
    \else\def\enddolines{\endhse}
    \fi
    \def\finishdolines{\end_hse}
   }

\def\hse{\begin_hse00}
\expandafter\def\csname hse*\endcsname{\begin_hse01}
\def\csp{\begin_hse10}
\expandafter\def\csname csp*\endcsname{\begin_hse11}

\let\beforehse=\beforeprs
\let\afterhse=\afterprs

\let\_oldstylenums=\oldstyle
\def\oldstyle{\numbersvar\oldstyle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


